Automated Penetration Testing: Formalization and Realization

Recent changes in standards and regulations, driven by the increasing importance of software systems in meeting societal needs, mandate increased security testing of software systems. Penetration testing has been shown to be a reliable method to asses software system security. However, manual penetration testing is labor-intensive and requires highly skilled practitioners. Given the shortage of cybersecurity experts and current societal needs, increasing the degree of automation involved in penetration testing can aid in fulfilling the demands for increased security testing. In this work, we formally express the penetration testing problem at the architectural level and suggest a general self-organizing architecture that can be instantiated to automate penetration testing of real systems. We further describe and implement a specialization of the architecture in the ADAPT tool, targeting systems composed of hosts and services. We evaluate and demonstrate the feasibility of ADAPT by automatically performing penetration tests with success against: Metasploitable2, Metasploitable3, and a realistic virtual network used as a lab environment for penetration tester training.

==> figures/CaseStudy.tex <==



==> figures/Discussion.tex <==
\subsection{Discussion}
\todo[]{This paragraph was moved here from the introduction}
\textcolor{red}{Automated penetration testing should ideally be (i) efficient, meaning that a test should be performed in a "smart" way to not waste resources, (ii) effective, i.e., able to cover at least the same/similar range of the target system that a human penetration tester would be able to, (iii) be able to deal with unknowns and uncertainties in dynamic systems, and (iv) generic, i.e., be applicable to multiple contexts without being redesigned and rebuilt from scratch.}

In terms of efficiency, the architecture is able to prioritize and pick targets and  attacks based on a set of utility concerns. Thus, its decision making depends the utility concerns and  their weights.
We selected our concerns and weights to prioritize exploiting deeper into the system using a combination of expert judgement and trial and error.  We have not extensively analyzed different parameter values, which we consider an interesting future work direction.
When it comes to effectiveness, our results show that the tool is able to 
to collect all flags in a non-trivial ethical hacking course.
Dynamicity and uncertainty are partially handled by the iterative nature of the MAPE-K loop that underpins our solution. Hosts that enter and leave the target system or interfaces enabled or disabled are identified by probes and post-exploitation scanners and considered in the next adaptation cycle. Nevertheless, since our case studies do not involve a high degree of dynamicity or uncertainty, the true extent of the implementation's capability to handle dynamicity and uncertainty is unclear.
In terms of generality, the tool is able to successfully exploit Metasploitable2, Metasploitable3 and the VM network utilizing the exact same attack and probe repertoires. The only difference between the tool invocations is the target IP range.

A few limitations of \toolname have to be noted. First, the process is not fully automated as the attack and probe repertoires need to be provided as tool input. Thus, using the tool shifts the main burden of work from manual tool running to attack and probe repertoire selection. It is important to consider the effort required to prepare the main inputs to the tool, i.e, to prepare and select the repertoires, the concerns and the associated utility functions and weights. 
Nevertheless, we can identify an improvement in terms of effort due to reuse and as the same attack and probe repertoires can be used to perform penetration testing on multiple systems with similar characteristics (architecture, domain, software stacks). Second, the tool contrary to
a human penetration tester is not able to identify novel attack patterns
or find new vulnerabilities. 



